A Ihara-Bass Formula for Non-Boolean Matrices and Strong Refutations of Random CSPs

We define a novel notion of ``non-backtracking'' matrix associated to any symmetric matrix, and we prove a ``Ihara-Bass'' type formula for it. We use this theory to prove new results on polynomial-time strong refutations of random constraint satisfaction problems with $k$ variables per constraints (k-CSPs). For a random k-CSP instance constructed out of a constraint that is satisfied by a $p$ fraction of assignments, if the instance contains $n$ variables and $n^{k/2} / \epsilon^2$ constraints, we can efficiently compute a certificate that the optimum satisfies at most a $p+O_k(\epsilon)$ fraction of constraints. Previously, this was known for even $k$, but for odd $k$ one needed $n^{k/2} (\log n)^{O(1)} / \epsilon^2$ random constraints to achieve the same conclusion. Although the improvement is only polylogarithmic, it overcomes a significant barrier to these types of results. Strong refutation results based on current approaches construct a certificate that a certain matrix associated to the k-CSP instance is quasirandom. Such certificate can come from a Feige-Ofek type argument, from an application of Grothendieck's inequality, or from a spectral bound obtained with a trace argument. The first two approaches require a union bound that cannot work when the number of constraints is $o(n^{\lceil k/2 \rceil})$ and the third one cannot work when the number of constraints is $o(n^{k/2} \sqrt{\log n})$. We further apply our techniques to obtain a new PTAS finding assignments for $k$-CSP instances with $n^{k/2} / \epsilon^2$ constraints in the semi-random settings where the constraints are random, but the sign patterns are adversarial.

==> content/bound-min-eigenvalue.tex <==
\section{Warm-up: spectrum of  binary matrices with dependencies}

In preparation to a proof of \cref{theorem:main}, we show here how to use the ideas of \cref{section:norm-bounds-via-ihara-bass} to study the spectrum of random  symmetric matrices with entries in $\Set{-1\,,0\,, 1}$, even when dependencies between the entries appear.
As we may view any symmetric matrix as the adjacency matrix of a weighted graph (up to the diagonal entries) we partially shift to the language of graphs. In particular, we study graphs sampled from the following family of distributions.

\begin{definition}[$\gamma$-wise independent random binary-weighted graphs]\label{definition:almost-independent-graph-distribution}
	$\cD_{d,\gamma}$ is the family of distributions $D_{d,\gamma}$ over graphs with vertex set $[n]$ with adjacency matrix satisfying:
	\begin{enumerate}
		\item for all $uv \in E(K_n)\,,$ $\bbP_{\mathbf{G}\sim D_{d,\gamma}} \Brac{A_{uv}(\mathbf{G})\neq 0 }=\bbP_{\mathbf{G}\sim D_{d,\gamma}} \Brac{uv\in E(\mathbf{G}) }=d/n\,.$
		\item for all $uv \in E(K_n)\,,$ the distribution of $A_{uv}(\mathbf{G})$ is symmetric with support $\{-1\,,0\,,+1\}\,.$
		\item the entries of $A(\mathbf{G})$ are $\gamma$-wise independent.%random variables $A_e(\mathbf{G}),\ldots w_{\mathbf{G}}(e_{\binom{n}{2}})$ 
	\end{enumerate}
\end{definition}
Notice that the adjacency matrix of $\mathbf{G}$ is a random binary matrix with $\gamma$-wise independent entries.
With a slight abuse of notation, we  write  $\mathbf{G}\sim \mathcal{D}_{d,\gamma}$ and $A(\mathbf{G})\sim\mathcal{D}_{d,\gamma}$, respectively for a graph sampled from $\mathcal{D}_{d,\gamma}$ and for its adjacency matrix. 
We consider the associated matrices $D(\mathbf{A})\,, B(\mathbf{A})$ as defined in \cref{section:general-ihara-bass}.
We prove the following theorem.

\begin{theorem}\label{theorem:main-binary}
	Let $n$ be an integer, $d>0$, $\gamma \geq O(\log^2 n)$\Tnote{\todo Check if tight} and consider a distribution $D_{d,\gamma}\in \cD_{d,\gamma}$. Then for $\mathbf{A}\sim \mathcal{D}_{d,\gamma}$,
	\begin{align*}
		\mathbf{A}\sge \Omega\Paren{-\sqrt{d}\cdot \Id_n + \frac{1}{\sqrt{d}}(D(\mathbf{A})-\Id_n)}
	\end{align*}
	with probability $1-o(1)$ (as $n\rightarrow \infty$).
\end{theorem}

The central tool behind \cref{theorem:main-binary} is the following lemma.

\begin{lemma}\label{lemma:radius-binary-non-backtracking}
	Let $n$ be an integer, $d>0$, $\gamma \geq O(\log^2 n)$\Tnote{Check if tight} and consider a distribution $D_{d,\gamma}\in \cD_{d,\gamma}$. Then for $\mathbf{A}\sim \mathcal{D}_{d,\gamma}$,
	\begin{align*}
		\rho\Paren{B(\mathbf{A})}\leq O(\sqrt{d})\,.
	\end{align*}
	with probability $1-o(1)$ (as $n\rightarrow \infty$).
\end{lemma}

Combining \cref{lemma:radius-binary-non-backtracking} with \cref{theorem:lowner-order-A} we immediately get \cref{theorem:main-binary}.  We will prove the Lemma via the trace method.

\begin{proposition}\label{proposition:trace-method}
	Let $\mathbf{M}$ be an $n$-by-$n$ random matrix and $c>0$. Then
	\begin{align*}
		\E_{\mathbf{M}}\Brac{\Tr \Paren{\mathbf{M}\transpose{\mathbf{M}}}^q}\leq \beta \Longrightarrow \bbP \Paren{\Norm{\mathbf{M}}\geq c\cdot \beta^{1/2q}}\leq c^{-2q}\,.
	\end{align*}
\end{proposition}

As we are not interested in the spectral norm of $B(\mathbf{A})$ --which may be large-- but in its spectral radius, we obtain first the following bound.

\begin{theorem}\label{theorem:spectrum-power-binary-non-backtracking}
	Let $n$ be an integer, $d>0$, $\gamma \geq \todo O(\log^2 n)$ and consider a distribution $D_{d,\gamma}\in \cD_{d,\gamma}$.  Let $ k\leq \frac{\log_d n}{10}$. Then for $\mathbf{A}\sim \mathcal{D}_{d,\gamma}$,
	\begin{align*}
		\Norm{B^{k-1}(\mathbf{A})}\leq O(d^{k/2})\cdot \polylog(n)\,.
	\end{align*}
	with probability $1-o(1)$ (as $n\rightarrow \infty$).
\end{theorem}

\cref{theorem:spectrum-power-binary-non-backtracking} implies \cref{lemma:radius-binary-non-backtracking} as a direct consequence.

\begin{proof}{Proof of \cref{lemma:radius-binary-non-backtracking}}
	Given \cref{theorem:spectrum-power-binary-non-backtracking}, it suffices to recall that by \cref{fact:bound-spectral-radius} for any integer $k\geq 1$
	\begin{align*}
		\rho(B(\mathbf{A}))\leq \Norm{B^k(\mathbf{A})}^{1/k}\,.
	\end{align*}
	Choosing $k\geq \Omega(\log_d n)$ the result follows.
\end{proof}

The rest of the section is devoted to the proof of \cref{theorem:spectrum-power-binary-non-backtracking}. In \cref{section:block-non-backtracking-matrices} we illustrate how the trace computation can be reduced to a path counting problem. In \cref{section:expectation-block-non-backtracking} we compute the expectation of such paths. Finally we put things together to prove \cref{lemma:radius-binary-non-backtracking} in \cref{section:proof-binary-theorem}.


\subsection{Powers of non-backtracking matrices}\label{section:block-non-backtracking-matrices}

%Our object of interest is thus the matrix $B(\mathbf{A})$, which we simply denote by $\mathbf{B}$.
For simplicity, we will simply write $B$ in place of $B(A)$ for an adjacency matrix $A$.
For a given non-backtracking matrix $B\in \R^{2m\times 2m}$, we consider the related matrix $B^*\in \R^{2n^2\times 2n^2}$ with entries
\begin{align*}
	B^*_{ef} = 
	\begin{cases}
		B_{ef}&\text{ if }e,f\in E(G)\\
		0&\text{ otherwise.}
	\end{cases}
\end{align*}
Recall here $G$ is the graph associated with $A$.
As eigenvalues and singular values of $B^*, B$ coincide (up to some additional zero-value ones). It suffices to study the spectrum of $B^*$. For this reason, we will henceforth denote  $B^*$ simply by $B$. The context will be clarified by the ambient dimension.



We now explain how to reduce the computation of the trace of powers of non-backtracking walks to a graph counting argument.
We start by introducing additional notions.
A graph $G$ is said $\ell$-\textit{tangle}-free if every neighborhood of radius $\ell$ in $H$ contains at most one cycle.
For a graph $G$ and $e,f \in \vec{E}(G)$, we write $\nbw{ef}{k}$ to denote the set of length $k$ non-backtracking walks in $G$ starting with $e$ and ending with $f$. 
Then $\nbw{}{k}(G) = \underset{e,f \in \vec{E}(G)}{\bigcup} \nbw{ef}{k}(G)$.
For simplicity we let $\nbw{ef}{k} := \nbw{ef}{k}(K_n)$.
We say that a walk $W\in \nbw{ef}{k}$ is tangle-free if the graph $G(W)= (V(W), E(W))$ is tangle-free.
We use $\tgf{ef}{k, \ell}(G)\subseteq \nbw{ef}{k}(G)$ to denote the subset of $\ell$-tangle-free walks.
We can extend the notion of closed non-backtracking matrices by introducing closed block non-backtracking matrices. $\bnbw{e}{q,k}$ is the set of walks $W$ of length $q\cdot k$ with starting edge $e\in \vec{E}(G)$ and ending edge $e^{-1}\in \vec{E}(G)$ satisfying:
\begin{enumerate}[(i)]
	\item $W$ can be partitioned into $k$ non-backtracking walks $W_1,\ldots, W_q$ of length $k$.
	\item For each pair of walks $W_{i}\,, W_{i+1}$ (with the convention $W_{q+1}=W_1$) the starting edge of $W_{i+1}$ is the inverse of the ending edge of $W_i$. I.e. we have $e_k(W_i) = e_1^{-1}(W_{i+1})$.
\end{enumerate}
Similarly, $\btgf{e}{q,k, \ell}\subseteq \bnbw{e}{q,k}$ is the set of closed block non-backtracking walks such that each block is $\ell$-tangle-free. If $\ell \geq k$ we simply write $\btgf{e}{q,k}$.
Given $W \in \bnbw{e}{q,k}$, we use $W_i\in \nbw{}{k}$ to denote the $i$-th block of $W$ (where the first block maybe chosen arbitrarily among  the ones starting at $e$). 

For a weighted graph $G$ (with possibly negative weights) with associated adjacency matrix $A\in \R^{n\times n}$ and an edge $uv\in E(G)\,,$ we write $\sigma_{uv}=\sign(A_{uv})$. Then for a oriented edge $e\in \vec{E}(G)$ we define
\begin{align*}
	\alpha_{e,s} = \begin{cases}
		\sigma_e& \text{if $s(e)\leq t(e)$}\\
		1& \text{otherwise.}
	\end{cases}
	\quad \text{and}\quad
		\alpha_{e,t} = \begin{cases}
		\sigma_e& \text{if $t(e)\leq s(e)$}\\
		1& \text{otherwise.}
	\end{cases}
\end{align*}

This notation will be used to describe the $k$-th power of the non-backtracking matrix.

\begin{fact}\label{fact:expansion-power-non-backtracking-matrix}
	Let $G$ be a weighted graph with $m$ edges. Let $A\in \R^{n\times n}$ be its adjacency matrix and $B\in \R^{2n^2\times n^2}$ the associated non-backtracking matrix.
	Let $e,f \in \vec{E}(G)$ and let $k$ be a positive integer. Then
	\begin{align*}
		(B^k)_{ef} = \sum_{W\in \nbw{ef}{k+1}}\alpha_{e,s}\cdot \alpha_{e,t} \cdot \sqrt{\Abs{A_{e_1}\cdot A_{e_{k+1}}}}\cdot \prod_{s=1}^{k-1}A_{e_{s+1}}\,.
	\end{align*}
\end{fact}

\cref{fact:expansion-power-non-backtracking-matrix} can be checked simply by expanding $B^k$. It will be convenient to decompose the sum as follows
\begin{align*}
	(B^k)_{ef} =& \sum_{W\in \nbw{ef}{k+1}}\alpha_{e,s}\cdot \alpha_{e,t} \cdot \sqrt{\Abs{A_{e_1}\cdot A_{e_{k+1}}}}\cdot \prod_{s=1}^{k-1}A_{e_{s+1}}\\
	=& \sum_{W\in \tgf{ef}{k+1}}\alpha_{e,s}\cdot \alpha_{e,t} \cdot \sqrt{\Abs{A_{e_1}\cdot A_{e_{k+1}}}}\cdot \prod_{s=1}^{k-1}A_{e_{s+1}} \\
	&+ \sum_{W\in \nbw{ef}{k+1}\setminus\tgf{ef}{k+1}}\alpha_{e,s}\cdot \alpha_{e,t} \cdot \sqrt{\Abs{A_{e_1}\cdot A_{e_{k+1}}}}\cdot \prod_{s=1}^{k-1}A_{e_{s+1}}\,.
\end{align*}
We write 
\begin{align*}
	(T^k)_{ef}:= \sum_{W\in \tgf{ef}{k+1}}\alpha_{e,s}\cdot \alpha_{e,t} \cdot \sqrt{\Abs{A_{e_1}\cdot A_{e_{k+1}}}}\cdot \prod_{s=1}^{k-1}A_{e_{s+1}}\,.
\end{align*}
Notice that for a $k$-tangle-free graph, $B^k=T^k\,.$ The trace of powers of $B^{k-1}$ can also be written as a sum over block non-backtracking walks.
 
\begin{fact}\label{fact:trace-expansion-non-backtracking-power}
	Let $G$ be a weighted graph with $m$ edges. Let $A\in \R^{n\times n}$ be its adjacency matrix and $B\in \R^{2n^2\times 2n^2}$ the associated non-backtracking matrix. Let $q, k\geq 2$ be integers. Then 
	\begin{align*}
		\Tr \Brac{B^{k-1}\transpose{\Paren{B^{k-1}}}}^q = \sum_{W\in \bnbw{}{2q,k}} \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{A_{e_1(W_i)}\cdot A_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}A_{e_{s+1}(W_i)}}}
	\end{align*}
\end{fact}

\subsection{Expectation of block non-backtracking walks}\label{section:expectation-block-non-backtracking}

By \cref{proposition:trace-method} and \cref{fact:trace-expansion-non-backtracking-power} we need to  study the expectation of closed block non-backtracking walks under distributions in $\cD_{d, \gamma}$. First we observe that, if an edge in a walk in $\bnbw{}{2q,k}$ has multiplicity one, then by symmetry the expectation of the whole walk is $0$. \Tnote{can be strengthen using odd moments in general}

\begin{fact}
	Let $n$ be an integer, $d>0\,,$ and $0<\gamma\leq n$. Consider a distribution $D_{d, \gamma}\in \cD_{d,\gamma}$.
	Let $W\in \bnbw{}{2q,k}$ with $k>1$ and $2q\cdot f\leq \gamma$. If there exists $e\in E(W)$ with multiplicity $m_W(e)=1$, then
	\begin{align}
		\E_{\mathbf{A}\sim D_{d, \gamma}} \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}}=0\,.
	\end{align}
	\begin{proof}
		By assumption there must be $e\in E(W)$ with $m_W(e)=1$ and by construction this cannot be any of the starting edges $e_{t\cdot k+1}$, with $0\leq t\leq 2q-1$ in $W$. 
		Let's denote this edge by $f\in \E(W)$.
		Then we may write
		\begin{align*}
		\E_{\mathbf{A}\sim D_{d, \gamma}}& \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}} \\
		&= \E_{\mathbf{A}\sim D_{d, \gamma}} \Brac{\prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}}\cdot \frac{1}{\mathbf{A}_{f}}}\cdot \E_{\mathbf{A}\sim D_{d, \gamma}}  \mathbf{A}_{f}\,,
		\end{align*}
		where we used $\gamma$-wise independence of the edges.
		By symmetry of the distribution $\E  \mathbf{A}_{f}=0$. The result follows.
	\end{proof}
\end{fact}

We say that a tangle-free walk $W\in \btgf{}{2q,k}$ is \textit{interesting} if there is no edge in $W$ with multiplicity one. We denote the set of interesting walks in $\btgf{}{2q,k}$ by $\ibtgf{}{2q,k}$. The next fact bounds the expectation of interesting closed block non-backtracking walks.

\begin{fact}\label{fact:expectation-binary-block-nbw}
	Let $n$ be an integer, $d>0\,,$ and $0<\gamma\leq n$. Consider a distribution $D_{d, \gamma}\in \cD_{d,\gamma}$.
	Let $W\in \ibtgf{}{2q,k}$ with $k>1$ and $2q\cdot f\leq \gamma$. Then
	\begin{align*}
		\E_{\mathbf{A}\sim D_{d, \gamma}} \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}} \leq \Paren{\frac{d}{n}}^{\Card{E(W)}}\,.
	\end{align*}
	\begin{proof}
		By $\gamma$-wise independence,
		\begin{align*}
			\E_{\mathbf{A}\sim D_{d, \gamma}} \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}} &\leq \prod_{e\in E(W)} \E_{\mathbf{A}\sim D_{d, \gamma}} \Abs{\mathbf{A}_{e}}^{m_W(e)}\\
			&=\prod_{e\in E(W)}  \E_{\mathbf{A}\sim D_{d, \gamma}}  \Abs{\mathbf{A}_{e}}\\
			&=\prod_{e\in E(W)} \Paren{\frac{d}{n}}\,.
		\end{align*}
	\end{proof}
\end{fact}

\subsection{Bound on the spectrum of non-backtracking matrices}\label{section:proof-binary-theorem}

We are ready to tackle \cref{theorem:spectrum-power-binary-non-backtracking}. Our proof consists of two main ingredients.
First we shows that, for a wide range of parameters, graphs sampled from distributions in $\cD_{d, \gamma}$ are tangle-free. Then we prove that the number of closed, tangle-free, block non-backtracking walks is not large. Combining these results with
\cref{fact:expectation-binary-block-nbw} will conclude the proof.


\begin{lemma}[Sparse graphs are tangle-free]\label{lemma:tangle-free-sparse-graph}
	Let $n$ be an integers. Let  $d>0$, $\log_d^2 n\leq \gamma\leq n$ and $\ell$ be such that $O(d^\ell)\leq \sqrt{\gamma}$\Tnote{Check if we need square root}. Consider a distribution $D_{d, \gamma}\in \cD_{d,\gamma}$.
	Then $\mathbf{G}\sim D_{d,\gamma}$ is $O(d^\ell)$-tangle-free with probability at least $1-o(1)$ (as $n\rightarrow \infty$).
	\begin{proof}
		For $v\in V(\mathbf{G})$ denote by $\mathbf{N}_\ell(v)$ the  $\ell$-neighborhood of $v$ in $\mathbf{G}$. We simply write that $\mathbf{G}$ is tangled in place of $\mathbf{G}$ is $O(d^\ell)$-tangled.
		By \Tnote{\todo in the appendix} $\E \Card{\mathbf{N}^2_\ell(v)}\leq O(d^{2\ell})$.
		Now 
		\begin{align*}
			\bbP \Paren{\mathbf{N}_\ell(v)\text{ is tangled}} =& \E \iverson{\mathbf{N}_\ell(v)\text{ is tangled}} \\
			\leq& \Paren{\frac{d}{n}}^2\cdot \E\Brac{ \Card{\mathbf{N}_\ell(v)}^2\given  \Card{\mathbf{N}_\ell(v)}\leq \sqrt{\gamma}} \\
			&+ \E\Brac{ \Card{\mathbf{N}_\ell(v)}^2\given  \Card{\mathbf{N}_\ell(v)}>\sqrt{\gamma}}\bbP \Paren{\Card{\mathbf{N}_\ell(v)}>\sqrt{\gamma}} \\
			\leq& \Paren{\frac{d}{n}}^2\cdot O(d^{2\ell})\,,
		\end{align*}
		where in the last step we used \Tnote{tail probability bound}.
		We can now apply Markov's inequality
		\begin{align*}
			\bbP \Paren{\mathbf{G}\text{ is tangled}}\leq \sum_{v\in [n]} \E \iverson{\mathbf{N}_\ell(v) \text{ is tangled}}\leq O\Paren{d^{2\ell+2}\cdot n^{-1}} =o(1)\,.
		\end{align*}
	\end{proof}
\end{lemma}

The fact that our graphs of interest are with high probability tangle-free means we need only to focus on this small subset of closed block non-backtracking walks.

We say that a walk $W\in \ibtgf{}{2q,k}$ is \textit{canonical} if for each edge $e\in E(W)$:
\begin{enumerate}[(i)]
	\item  $s(e)< t(e)$,  that is the source of the label vertex is smaller than the label of the target vertex.
	\item $s(e) = t(e)-1$, i.e. the two label are consequential.
\end{enumerate}
The use of canonical paths is convenient as, by construction, no two canonical paths are isomorphic (so we are in fact choosing an arbitrary element for each equivalence class). We denote the set of canonical paths by $\cW^{2q,k}\subseteq\ibtgf{}{2q,k}$. Notice that for $P \in \cW^{2q,k}$, there are $\binom{n}{v}(v)!$ isomorphic walks in $\ibtgf{}{2q,k}$.

\begin{lemma}[Enumeration of canonical paths, \cite{BordenaveLM15} Lemma $17$ ]\label{lemma:enumeration-binary-canonical-paths}
	Let $\cW^{2q,k}(v,e)$ be the set of canonical paths with $v$ vertices and $e$ distinct edges. We have
	\begin{align*}
		\Card{\cW^{2q,k}(v,e)}\leq k^{2q}\cdot (2kq)^{6q\cdot (e-v+1)}\,.
	\end{align*}
\end{lemma}


We are now ready to prove the theorem.

\begin{proof}[Proof of \cref{theorem:spectrum-power-binary-non-backtracking}]
	First notice that by \cref{lemma:tangle-free-sparse-graph}
	\begin{align*}
		\E&\Brac{ \Tr \Brac{\mathbf{B}^{k-1}\transpose{\Paren{\mathbf{B}^{k-1}}}}^q \given \mathbf{G} \text{ is tangle-free}} \\
		&= \sum_{W\in \ibtgf{}{2q,k}} \E \Brac{\prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}}\given \mathbf{G} \text{ is tangle-free}}\\
		&\leq O\Paren{  \sum_{W\in \ibtgf{}{2q,k}} \E \prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}}}\,.
	\end{align*}
	Now by \cref{fact:expectation-binary-block-nbw} and \cref{lemma:enumeration-binary-canonical-paths}
	\begin{align*}
		\sum_{W\in \ibtgf{}{2q,k}} \E &\prod_{i=1}^{2q}\Brac{ \sqrt{\Abs{\mathbf{A}_{e_1(W_i)}\cdot \mathbf{A}_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\mathbf{A}_{e_{s+1}(W_i)}}}\\
		&\leq 	\sum_{W\in \ibtgf{}{2q,k}} \Paren{\frac{d}{n}}^{E(W)}\\
		&\leq \sum_{v\geq 3}^{k\cdot q+1}\sum_{e=v-1}^{k\cdot q}\Card{\cW^{2q,k}(v,e)}\cdot \binom{n}{v}(v)!\cdot \Paren{\frac{d}{n}}^e\\
		&\leq  \sum_{v\geq 3}^{k\cdot q+1}\sum_{e=v-1}^{k\cdot q} (3\cdot n)^{v} \cdot k^{2q}\cdot (2kq)^{6q\cdot (e-v+1)}\cdot \Paren{\frac{d}{n}}^e\\
		&\leq \sum_{v\geq 3}^{k\cdot q+1}\sum_{e=v-1}^{k\cdot q}k^{2q}\cdot d^{e}\cdot n\cdot  \Paren{\frac{(6kq)^{6q}}{n}}^{e-v+1}\\
		&\leq k^{2q}\cdot d^{kq}\cdot n\cdot\sum_{v\geq 3}^{k\cdot q+1}\sum_{e=v-1}^{k\cdot q}  \Paren{\frac{(6kq)^{6q}}{n}}^{e-v+1}\,.
	\end{align*}
	For $q=\frac{\log n}{10\log\log n}$ and $k\leq \frac{\log_d n}{6}$\Tnote{Double check} the series converge.
	Thus
	\begin{align*}
		\E\Brac{ \Tr \Brac{\mathbf{B}^{k-1}\transpose{\Paren{\mathbf{B}^{k-1}}}}^q \given \mathbf{G} \text{ is tangle-free}}  &\leq O\Paren{k^{2q}\cdot d^{kq}\cdot n}
	\end{align*}
	Finally by \cref{proposition:trace-method} with probability at least $1-o(1)$
	\begin{align*}
		\Norm{\mathbf{B}^k}\leq O(d^{k/2})\cdot \Paren{k^2\cdot n^{1/q}}\leq  O(d^{k/2})\cdot \polylog(n)\,,
	\end{align*}
	concluding the proof.
\end{proof}


%\begin{lemma}
%	Let $G$ be $O(\polylog(n))$-tangle-free with probability $1-p$ \Tnote{and log-n wise independence, define $\ibtgf{arg1}{arg2}$}. Then
%	\begin{align*}
%		\E \Tr \Brac{B^{k-1}\transpose{\Paren{B^{k-1}}}}^q \leq \frac{1}{1-p} \sum_{W\in \ibtgf{}{2q,k}} \prod_{i=1}^{2q}\Brac{\E\sqrt{\Abs{A_{e_1(W_i)}}}\cdot\E \sqrt{\Abs{ A_{e_k(W_i)}}}\cdot\Paren{\prod_{s=2}^{k-1}\E A_{e_{s+1}(W_i)}}}\,.
%	\end{align*}
%\end{lemma}






==> content/cut-norm-bound.tex <==
\section{Spectrum bounds via the Ihara-Bass formula}

In this section we show how \cref{theorem:general-ihara-bass} can be used to study the spectrum of a real symmetric matrix $A$ via of the spectrum of related matrices.


\begin{theorem}\label{theorem:lowner-order-A}
	Let $A\in \R^{n\times n}$ a  symmetric matrix. Let $B\,, L\,, J\,, D$ be as defined in \cref{section:general-ihara-bass}. Let $\lambda_{\min}$ be the smallest eigenvalue of the matrix $B+L-J\in \R^{2m\times 2m}$. Then
	\begin{align*}
		A \sge - \Abs{\lambda_{\min}}\Id_n  +\Paren{\Abs{\lambda_{\min}}}^{-1}(D-\Id_n)\,.
	\end{align*}
	\begin{proof}
		\Tnote{The argument described by Luca}
	\end{proof}
\end{theorem}

A crucial consequence of \cref{theorem:lowner-order-A} is that, exploiting the diagonal structure of the matrices $D\,,\Id_n$ one can easily bound the cut-norm of the matrix $A$.

\begin{corollary}
	Consider the settings of \cref{theorem:lowner-order-A}. Then
	\begin{align*}
		\Normc{A}\leq  \Abs{\lambda_{\min}}^{-1} \cdot \Normc{D-(1+\Abs{\lambda_{\min}}^2)\cdot\Id_n} \,.
	\end{align*}
\end{corollary}



==> content/cut-norm-xor.tex <==
\section{Refutation for random 3-xor}\label{section:random-3xor}

Let $T\in (\R^n)^{\otimes 3}$ be a random  a random symmetric $3$-tensor with distributionally independent entries such that for distinct $a,b,c\in [n]$
\begin{align*}
	T_{a,b,c} = \begin{cases}
		0& \text{with probability }1-p\,,\\
		+1&\text{with probability }p/2\,,\\
		-1&\text{with probability }p/2\,.
	\end{cases}
\end{align*}

In this section we aim to prove the following result.

\begin{theorem}\label{theorem:cut-norm-A}
	Let $\mathbf{T}$ be a $3$-order tensor as in \todo and suppose $p\geq n^{-1.5}$. Let $\epsilon(n)=\todo$
	Consider the $n^2$-by-$n^2$ matrix
	\begin{align*}
		\mathbf{A}_{(a,b),(c,d)}:= \sum_{\ell\in [n]}\mathbf{T}_{a,c,\ell}\cdot \mathbf{T}_{b,d,\ell}\,.
	\end{align*}
	Then 
	\begin{align*}
		\Normg{\mathbf{A}}\leq O\Paren{\eps^2\cdot p^2\cdot n^5}
	\end{align*}
	with probability $1-o(1)$.
\end{theorem}


We may rewrite $\mathbf{A}=\mathbf{A}'+\mathbf{A}''$ where 
\begin{align}\label{eq:preprocessed-A}
		\mathbf{A}'_{(a,b),(c,d)}:= 
		\begin{cases}
			\mathbf{A}_{(a,b),(c,d)}& \text{if }\Set{a,c}\cap\Set{b,d}=\neq \emptyset\\
			0&\text{ otherwise}
		\end{cases}
\end{align}
and $\mathbf{A}''=\mathbf{A}-\mathbf{A}'$. By triangle inequality, to prove \cref{theorem:cut-norm-A} it suffices to bound the norm $\normg{\cdot}$ of both $\mathbf{A}'$ and $\mathbf{A}''$, which we do next.

\begin{lemma}\label{lemma:cut-norm-preprocessed-A}
	Consider the settings of \cref{theorem:cut-norm-A}.
	Let $\mathbf{A}'$ as defined in \cref{eq:preprocessed-A} 
	Then with probability $1-n^{-\Omega(1)}$ 
	\begin{align*}
		\Normg{\mathbf{A}'}\leq O(\eps^2\cdot p^2\cdot n^5)\,.
	\end{align*}
\end{lemma}

We prove \cref{lemma:cut-norm-preprocessed-A} in \cref{section:bounding-norm-preprocessed-A} and focus here on $\mathbf{A}''$.

\begin{lemma}\label{lemma:cut-norm-residual-A}
	Consider the settings of \cref{theorem:cut-norm-A}. 
	Let $\mathbf{A}'$ as defined in \cref{eq:preprocessed-A} and let $\mathbf{A}''= \mathbf{A}-\mathbf{A}'$.
	Then with probability $1-o(1)$ 
	\begin{align*}
		\Normg{\mathbf{A}''}\leq O(p^2\cdot n^{4.9})\,.
	\end{align*}
	\begin{proof}
		Since each entry in $\mathbf{A}''$ is either zero or larger than $1$ in absolute value, we have $\Normg{\mathbf{A}''}\leq \Snorm{\mathbf{A}''}_F$.
		We may decompose $\Normf{\mathbf{A}''}^2$ as
		\begin{align*}
			\Normf{\mathbf{A}''}^2 =& \sum_{a,b\in [n]}\Brac{ \Paren{\mathbf{A}''_{(a,b),(b,a)}}^2 + \Paren{\mathbf{A}''_{(a,a),(b,b)}}^2}\\
			&+  \sum_{\substack{a,b,c\in [n]\\a\neq c}} \Brac{\Paren{\mathbf{A}''_{(a,c),(b,b)} }^2+\Paren{\mathbf{A}''_{(b,b)(a,c)}}^2+\Paren{\mathbf{A}''_{(b,a)(c,b)}}^2+\Paren{\mathbf{A}''_{(a,b)(b,c)}}^2}\,.
		\end{align*}
		We first bound $\sum_{a,b\in [n]} \Paren{\mathbf{A}''_{(a,b),(b,a)}}^2$. To this end notice that for any $t\geq 1\,,$ and $a,b \in [n]$
		\begin{align*}
			\bbP \Paren{\Paren{\mathbf{A}''_{(a,b),(b,a)}}^2=t^2}&= \bbP \Paren{\Paren{\sum_{\ell\in[n]}T_{a,b,\ell}^2}^2=t^2} = \\
			&= \bbP \Paren{\Abs{\sum_{\ell\in[n]}T_{a,b,\ell}^2}=t} \\
			&\leq \binom{n}{t}(1-p)^{n-t}p^t\\
			&\leq \binom{n}{t}p^t\\
			&\leq \Paren{\frac{e\cdot n\cdot p}{t}}^t\,.
		\end{align*}
		%Consider the following function $f:\Z_+\rightarrow \R_+$ with $f(1)=100/p^{1/10}$ and $f(t)=2^tf(1)$. For fixed $t\geq 1$ by Markov's inequality:
		We split the contribution of entries based on their magnitude and bound their number using Markov's inequality. For any $t\geq 1$, denote by $\cE_t$ the event that 
		\[\sum_{a,b\in [n]} \Paren{\mathbf{A}''_{(a,b),(b,a)}}^2\iverson{\mathbf{A}''_{(a,b),(b,a)}=t}\leq 100\cdot n^2 \cdot p^{1/10}\cdot 2^{-t}
		\]
		and let $\bar{\cE}_t$ be its complement. 
		Notice that if $\cE_t$ is verified for all $t\geq 1$, then
		\begin{align*}
			\sum_{a,b\in [n]} \Paren{\mathbf{A}''_{(a,b),(b,a)}}^2\leq 10^3\cdot n^2\cdot p^{1/10}\leq O(p^2\cdot n^{4.9})\,,
		\end{align*}
		where in the last step we used the assumption that $p\geq n^{-1.5}$. We  verify that with high probability this intersection event happens.	By Markov's inequality
		\begin{align*}
			\bbP \Paren{\bar{\cE}_t}\leq \Paren{2e\cdot n \cdot p}^t\cdot \frac{100}{p^{1/10}}\,.
		\end{align*}
		Thus 
		\begin{align*}
			\bbP \Paren{\underset{t\geq 1}{\bigcup}\bar{\cE}_t}\leq O(n\cdot p^{9/10})\leq n^{-\Omega(1)}\,.
		\end{align*}
		As $\sum_{a,b\in [n]} \Paren{\mathbf{A}''_{(a,q),(b,b)}}^2$ can be bounded analogously, we focus next on  $\sum_{\substack{a,b,c\in [n]\\a\neq c}} \Paren{\mathbf{A}''_{(a,c),(b,b)}}^2$.
		For fixed and distinct $a,b,c\in [n]$
		\begin{align*}
			\E \Brac{\Paren{\mathbf{A}''_{(a,c),(b,b)}}^2} &= \sum_{\ell, \ell'\in [n]}\E \mathbf{T}_{a,b,\ell}\mathbf{T}_{c,b,\ell}\mathbf{T}_{a,b,\ell'}\mathbf{T}_{c,b,\ell'}\\
			&= \sum_{\ell\in [n]}\E \mathbf{T}_{a,b,\ell}^2\mathbf{T}_{c,b,\ell}^2\\
			&\leq np^2\,,
		\end{align*}
		where in the second step we used independence of the entries of $\mathbf{T}$.
		By Markov's inequality
		\begin{align*}
			\bbP \Paren{\sum_{\substack{a,b,c\in [n]\\a\neq c}} \Paren{\mathbf{A}''_{(a,c),(b,b)}}^2\geq t\cdot n^3}\leq \frac{np^2}{t}\,.
		\end{align*}
		Choosing $t= n^{1.1}p^2$ and repeating this second analysis for the remaining terms the result follows.
	\end{proof}
\end{lemma}


\subsection{Bounding the norm of A'}\label{section:bounding-norm-preprocessed-A}

To prove \cref{lemma:cut-norm-preprocessed-A} we use \cref{theorem:general-ihara-bass}. 
In particular, we prove the result below.

\begin{theorem}\label{theorem:bound-preporcessed-A-via-Ihara-Bass}
	Consider the settings of \cref{lemma:cut-norm-preprocessed-A}. Let $\mathbf{B}, \mathbf{L}, \mathbf{D}$ be the matrices associated to $\mathbf{A}'$ as defined in \cref{section:general-ihara-bass}.
	Then with probability $1-o(1)$
	\begin{align*}
		\rho(\mathbf{B}+\mathbf{L}-\mathbf{D})\leq \todo\,.
	\end{align*}
\end{theorem}

\Tnote{Proof of \cref{lemma:cut-norm-preprocessed-A} here.}

By definition of spectral radius, there exists some unit vector $v\in \R^m$ such that
\begin{align*}
	\rho(\mathbf{B}+\mathbf{L}-\mathbf{J})\leq \transpose{v}(\mathbf{B}+\mathbf{L}-\mathbf{J})v\leq \rho(\mathbf{B})+ \Norm{\mathbf{L}}+ \Norm{\mathbf{J}}.
\end{align*}
Thus, we can use next two results to obtain \cref{theorem:bound-preporcessed-A-via-Ihara-Bass}.

\begin{lemma}
	Consider the settings of \cref{theorem:bound-preporcessed-A-via-Ihara-Bass} and suppose $p\leq n^{-1}$. Then with probability $1-o(1)$
	\begin{align*}
		\Norm{\mathbf{L}}+\Norm{\mathbf{J}}\leq O(1)\,.
	\end{align*}
	\begin{proof}
		By construction $\Norm{\mathbf{J}}\leq 1$ and  $\Norm{\mathbf{L}}\leq \max_{a,b,c,d\in [n]}\Abs{\mathbf{A}'_{(a,b)(c,d)}}$.
		Now, for fixed distinct $a,b,c,d\in [n]$ and $t\geq 1$
		\begin{align*}
			\bbP \Paren{\Abs{\mathbf{A}'_{(a,b)(c,d)}}\geq t} &= \bbP \Paren{\Abs{\mathbf{A}'_{(a,b)(c,d)}} \geq t}\\
			%&=\sum_{q\geq t}\bbP \Paren{\Paren{\mathbf{A}'_{(a,b)(c,d)}}^2 = q^2}\\
			%&=\sum_{q\geq t}\bbP \Paren{\Paren{\sum_{\ell\in[n]}T_{a,c,\ell}T_{b,d,\ell}}^2 = q^2}\\
			&= \bbP \Paren{\Abs{\sum_{\ell\in[n]}T_{a,c,\ell}T_{b,d,\ell}}\geq t}\\
			&=\bbP \Paren{\sum_{\ell\in[n]}\Abs{T_{a,c,\ell}T_{b,d,\ell}}\geq t}\\
			&\leq \sum_{q\geq t}\bbP \Paren{\sum_{\ell\in[n]}\Abs{T_{a,c,\ell}T_{b,d,\ell}}= q}\\
			&\leq \sum_{q\geq t} \binom{n}{q}\cdot p^{2q}\cdot (1-p)^{n-2q}\\
			&\leq  \sum_{q\geq t} \binom{n}{q}\cdot p^{2q}\\
			&\leq O(1)\cdot\Paren{\frac{e\cdot n\cdot p^2}{t}}^{t}	\,.
		\end{align*}
		Thus, as $p\leq n^{-1}$ and $\mathbf{A}''$ has $n^4$ entries, by union bound $\max_{a,b,c,d\in [n]}\Abs{\mathbf{A}'_{(a,b)(c,d)}}\leq 1000$, with probability  $1-n^{-\Omega(1)}$.
	\end{proof}
\end{lemma}

\begin{lemma}\label{lemma:spectral-radius-non-backtracking}
	Consider the settings of \cref{theorem:bound-preporcessed-A-via-Ihara-Bass}. Then with probability $1-o(1)$
	\begin{align*}
		\rho(\mathbf{B})\leq \todo.
	\end{align*}
\end{lemma}

The rest of the section is dedicated to proving \cref{lemma:spectral-radius-non-backtracking}.

